Test-optional Policies: Overcoming Strategic Behavior and Informational Gaps

Due to the Covid-19 pandemic, more than 500 US-based colleges and universities went "test-optional" for admissions and promised that they would not penalize applicants for not submitting test scores, part of a longer trend to rethink the role of testing in college admissions. However, it remains unclear how (and whether) a college can simultaneously use test scores for those who submit them, while not penalizing those who do not--and what that promise even means. We formalize these questions, and study how a college can overcome two challenges with optional testing: $\textit{strategic applicants}$ (when those with low test scores can pretend to not have taken the test), and $\textit{informational gaps}$ (it has more information on those who submit a test score than those who do not). We find that colleges can indeed do so, if and only if they are able to use information on who has test access and are willing to randomize admissions.

==> model_oldcopy.tex <==
\section{Model}
\label{sec:model}

Our model extends that of~\citet{garg2020standardized}, such that a test score can be optionally submitted. %

\parbold{Students. } There is a unit mass of students. Each student has a latent skill level $q$, normally distributed as $\mathcal{N}(\mu,\sigma^2)$, as well as a set of observed features $\Theta$. All students have the first $K-1$ features $\{1,\dots,{K-1}\}$; only a subset apply with the last feature $K$. For each student, $\theta_k$ is a noisy function of $q$, i.e., $\theta_k = q + \epsilon_k$, for $k = 1,\dots,K$, with Gaussian noise $\epsilon_k\sim \mathcal{N}(0,\sigma_k^2)$. The distribution of noise $\epsilon_k$ is feature dependent, but independent across features and students. Throughout our exposition, we refer to feature $K$ as the ``test score.'' 

For each student, let $Z, Y, X \in \{0, 1\}$ be indicators denoting whether the student has \textit{access} ($Z$) the test, \textit{takes} ($Y$) it, and reports their score ($X$), respectively. Of course, $Z \geq Y \geq X$. Access $Z$ is deterministic and pre-set, uncorrelated with $q$ and other features. Students with access ($Z=1$) may decide to take the test ($Y=1$), with full knowledge of their skill $q$, noise distribution $\epsilon_K$, other features $\{\theta_k\}_{k=1}^{K-1}$ for ${k < K}$, the school's policy $P$ (defined below)\zhi{students may not know all of $P$: it could be convenient if the selection process is not fully revealed.}, and the induced equilibrium (decisions and scores of other students). Students who take the test may, with knowledge of their test score $\theta_K$, decide to report it ($X=1$), in which case the school further observes their  score $\theta_K$. Students make these decisions to maximize their admissions probability. We denote the resulting decisions via the functions $Y(q, \{\theta_k\}_{k=1}^{K-1}, P)$ and $X(\{\theta_k\}_{k=1}^{K}, P)$, and note that these are random variables for each student, as they depend on random features $\theta_k$.\footnote{It is simple to see that $X$ should not depend on $q$, given $\theta_K$. Once the test score is sampled from the student's skill level, the student's admission probability does not depend on $q$.} We assume that the school knows the functions $Y(\cdot), X(\cdot)$, for example by observing the values distributionally over time. \todo{justify the functions being known}






\parbold{School. } \zhi{Updated here to specify $P$.}A single school admits a mass $C < 1$ of students, using an admission policy $P$ that is further divided into two part: an \textbf{estimation process} that maps the abailable information from each student to an estimated skill level, and an \textbf{selection process} that assigns a probability of admission to each student given the estimated skill. The two processes are cunducted as follows.

For each student, upon observing information set $I$, the school forms an \textit{estimate} $\tilde q$ of their skill level $q$ via an estimation function $f(I)$. For example, $I$ always contains $\{\theta_k\}_{k=1}^{K-1}$ and $X$ (whether the student reports a score); if $X=1$, it further includes $\theta_K$. 
In our baseline policy, the school calculates the posterior mean in a Bayesian optimal manner, using all the information available: %
$\tilde q = f(I) \triangleq \E[q | I]$. Note that this calculation is \textit{in equilibrium}; e.g., if every student with $q \geq 1$ reports their test score, then $\E[q | X = 0]$ will be less than $1$. \todo{clearer writing here} Unlike~\citet{garg2020standardized}, we further consider non-Bayesian optimal estimation policies $f$.%

After estimating skills, the school assigns a probability of admission based on the estimation by a selection function $g(\tilde{q})$. The school aims to admit a fraction $C$ overall, so the selection function is designed so that $\int_{-\infty}^{\infty}g(q)dq=C$. For example, if the school only wishes to admit the highest $C$ fraction of students, then $g(\cdot)$ would be exactly 1 for $\tilde{q}$ in the highest $C$ fraction of its distribution, and exactly 0 otherwise.\todo{unclear right now whether will need highest $C$ overall or also per group}. 

Let $A\in \{0,1\}$ indicate whether a student is admitted. 

\todo{Define $P$ as estimation + selection policy. }

\todo{write down what an equilibrium means}

\parbold{Equilibrium. }The admission policy and the strategy of students induce an equilibrium. We assume that the students strategize to maximize their probability of getting admitted, based on the extent of their knowledge. In equilibrium, no students have the incentive to opt out of their current decision, meaning that their current decision is optimal in terms of the resulting probability of admission, given knowledge known. Note that there may be ties: for some students, the two decisions (yes/no to reporting after taking the test, or yes/no to taking the test and report) might lead to the same probability of admission. So the equilibrium is only unique up to the set of students admitted. \zhi{or unique up to the probability of admissions for every student?} 

    









\subsection*{Objective metrics}
We will evaluate policies with respect to the following objectives. 
\textbf{{Academic merit}} is the expected skill level of the admitted class, $\E[q | A = 1]$. It is maximized by adopting a Bayesian optimal estimation policy and then admitting the fraction $C$ of students with the highest skill estimates. 

\parbold{What does test-optional mean?} Schools do not only care about academic merit as defined.\footnote{In practice, of course, many other objectives also matter, to produce a balanced college cohort~\cite{selingo2020whogetsin}.} Here, we consider the following ``fairness'' notions, meant to capture ways to formalize the pledge to  ``not penalize students for the absence of a standardized test score''~\cite{testoptional21}.

\begin{definition}[Latent skill fairness]
    \label{deffair1}
    An admissions policy is \textbf{latent skill fair} if for all $q$,
    $$
    \P\left[A=1|Z=1, q \right]=\P\left[A=1|Z=0, q\right].
    $$
\end{definition}

\begin{definition}[Observable fairness]
    \label{deffair2}
    An admissions policy is \textbf{observably fair} if for all $\{\theta_k\}_{k=1}^{K-1}$,
    $$
    \P\left[A=1|Z=1,\{\theta_k\}_{k=1}^{K-1}\right]=\P\left[A=1|Z=0,\{\theta_k\}_{k=1}^{K-1}\right].
    $$
\end{definition}

\nikhil{I added the following. it's weaker than 2.2 and holds when doing bayesian optimal estimation with affirmative action. same proofs of 2.2 not working with strategic agents should hold here }
\begin{definition}[Demographic fairness]
    \label{deffair2}
    An admissions policy is \textbf{demographically fair} if
    $$
    \P\left[A=1|Z=1\right]=\P\left[A=1|Z=0\right].
    $$
\end{definition}


\todo{Earlier language, need to edit:} We consider Observable fairness to be most aligned with reality. The claim of ``not punishing students'' because they do not have access to tests should mean that within the two cohorts, if their are two groups of students in each with the same features $\theta_1$ to $\theta_{K-1}$, then they should have, in expectation, the same probability of getting admitted. This claim agrees with \ref{deffair2}, hence we mainly focus on this criterion in later discussions. \todo{should we explain this here in more detail, or explain it somewhere else, or add something in later parts addressing the other criteria?} \nikhil{good question. Unclear how we want to present the definitions and assumptions.}

\todo{Discuss these notions more}

Finally, note that a school can trivially achieve these notions by ignoring test scores (both the student's score $\theta_K$ and whether they submitted the test $X$) altogether.

\begin{definition}[Test blank]
    An admissions policy is \textbf{test blank}, i.e., it ignores the test score, if
    \begin{align*}
        \P\left[A=1|\{\theta_k\}_{k=1}^{K-1}\right]&=\P\left[A=1|\{\theta_k\}_{k=1}^{K-1},\theta_K\right] &\forall \  \{\theta_k\}_{k=1}^{K}\\
        \equiv \P\left[A=1|X=1,\{\theta_k\}_{k=1}^{K-1}\right]&=\P\left[A=1|X=0,\{\theta_k\}_{k=1}^{K-1}\right]. &\forall \  \{\theta_k\}_{k=1}^{K-1}
    \end{align*}
\end{definition}

However, ignoring test scores altogether might both hurt the school's academic merit goals and be especially harmful for students without access to other informative signals with which to distinguish themselves~\cite{garg2020standardized}.  

\todo{Think about fairness conditioned on $X$ as well? if that's what we do in Section 4, then include that here. Also maybe bring back that notion I commented out for now }
